Max-Quantile Grouped Infinite-Arm Bandits

In this paper, we consider a bandit problem in which there are a number of groups each consisting of infinitely many arms. Whenever a new arm is requested from a given group, its mean reward is drawn from an unknown reservoir distribution (different for each group), and the uncertainty in the arm's mean reward can only be reduced via subsequent pulls of the arm. The goal is to identify the infinite-arm group whose reservoir distribution has the highest $(1-\alpha)$-quantile (e.g., median if $\alpha = \frac{1}{2}$), using as few total arm pulls as possible. We introduce a two-step algorithm that first requests a fixed number of arms from each group and then runs a finite-arm grouped max-quantile bandit algorithm. We characterize both the instance-dependent and worst-case regret, and provide a matching lower bound for the latter, while discussing various strengths, weaknesses, algorithmic improvements, and potential lower bounds associated with our instance-dependent upper bounds.

==> finite_arm.tex <==
\label{sec:finite}

\red{Our finite-arm subroutine, \texttt{FiniteArmBQID}, and its analysis will be generally similar to the main algorithm in \cite{wang2021max}, though with different details.
Their algorithm can be viewed as taking $\alpha = 1$ and $\Delta = 0$ in our notation, whereas we are interested in an \textit{arbitrary} $\alpha \in (0,1)$ and we allow for $\Delta$ to be positive.  Moreover, in \cite{wang2021max} the groups are allowed to overlap; we avoided such considerations because they seem tricky to formulate neatly in the infinite-arm setting, but in the finite-arm setting of this section it would be straightforward to incorporate.
However, we emphasize that the key distinction is not these details, but rather the challenges of
incorporating the finite-arm algorithm into an infinite-arm framework.}

% In this section, we formally define our choice of \texttt{FiniteArmBQID} used 
% in Line~5 of Algorithm~\ref{alg:main}.  Recall that in Section \ref{sec:num_pulls} we introduced the high-level ideas and fundamental gaps associated with our choice of this subroutine.  The details are perhaps most similar to \cite{wang2021max}, in particular using a successive elimination approach.\footnote{We expect that other approaches such as LUCB-type algorithms could also provide similar guarantees.  However, see Appendix \ref{sec:structured} for a discussion on how an existing LUCB-based bound for a general structured bandit framework can be weaker than ours.}  The algorithm in \cite{wang2021max} can be viewed as taking $\alpha = 1$ and $\Delta = 0$ in our notation, whereas we are interested in $\alpha \in (0,1)$ and we allow for $\Delta$ to be positive.  Moreover, in \cite{wang2021max} the groups are allowed to overlap; we avoided such considerations because they seem tricky to formulate neatly in the infinite-arm setting, but in the finite-arm setting of this section it would be straightforward to incorporate.

%and allow overlaps between groups but assumes there is a unique optimal group. In contrast, our scheme allows $0 < \alpha, \Delta \le 1$ and multiple optimal groups, but allows no overlaps between groups (though it can be easily adapted). We believe this algorithm is of interest in its own right.

% {\color{red} [TODO: This might not flow well given that we already sort of covered elimination in Section \ref{sec:num_pulls}]}
% Elimination-based algorithms are widely used in MAB problems, especially in the standard best-arm identification setting.
% The rough idea is to keep looping the following three steps until some stopping criterion is satisfied: (i) pull all arms that are not yet eliminated; (ii) update their confidence bounds based on observed rewards; (iii) eliminate arms known to be suboptimal based on confidence bounds.  In the setting that we consider, we can use a similar idea, but we need to carefully consider the conditions under which an arm no longer needs to be pulled. 
% We proceed by describing this and giving the relevant definitions.

A complete description of our finite-arm subroutine will be given in Algorithm~\ref{alg:elimination} in Appendix~\ref{sec:se}, with its analysis  in Appendix~\ref{sec:appendix_finite_alg}.  
The algorithm  uses a successive elimination approach,\footnote{We expect that other approaches such as LUCB-type algorithms could also provide similar guarantees.  However, see Appendix \ref{sec:structured} for a discussion on how an existing LUCB-based bound for a general structured bandit framework can be weaker than ours.}
by maintaining a set of ``active'' arms and groups throughout
% that will be pulled in the next round 
(see \eqref{def:C_t}, \eqref{def:m_t}, \eqref{def:B_t}, and Lines~\ref{line:update_C_t}-\ref{line:update_B_t} of Algorithm~\ref{alg:elimination}).
At each round, the algorithm pulls all arms in the set of active arms, updates their confidence bounds, and eliminates groups that are suboptimal and arms that are ``no longer of interest'' based on the confidence bounds.
When the algorithm identifies that
% only one active group remains, or 
some group satisfies 
\eqref{eq:optimal H} based on the confidence bounds, it terminates and returns that group.
% identifies a group that satisfies \eqref{eq:optimal H} with high probability.

% \red{While the algorithm and results in this section are used as a stepping stone to the overall guarantees of Algorithm \ref{alg:main}, we believe that they are also of interest in their own right. (remove so that (25) appears in page 12?)}




==> kauffman.tex <==
\subsection{Setup, Assumptions, and Notation}\label{setup}

Let $(\Arms, \ArmEvents, \ArmMeasure)$ be a probability space over arms
with measure $\ArmMeasure$,
where each arm $\arm \in \Arms$ is some abstract object (e.g. a classifier),
and let $(\ExpRewards, \ExpRewardEvents)$ be a measurable space over
expected rewards, where $\ExpRewards \subseteq \R$ is a
continuous interval
and $\ExpRewardEvents$ is the Borel $\sigma$-algebra over $\ExpRewards$
(i.e. the smallest $\sigma$-algebra containing all sub-intervals of $\Theta$).
Also let
$P_{\ExpRewards} = \Set{ p_{\expReward}, \expReward \in \ExpRewards }$
be a parametric set of probability distributions such that each
distribution is continuously parameterized by its mean.
To ease the notation, we shall assume
%\begin{align*}
$\ENone_{X \sim p_{\expReward}}[X] = \expReward$.
%\end{align*}
One can think of $P_{\ExpRewards}$ as a one-parameter exponential family (e.g. the
family of Bernoulli, Gaussian with fixed and known variance, Poisson or Exponential distributions with means
in some interval or other subset of $\R$),
however we do not limit ourselves to such well-behaved reward distributions.
% We defer our further assumptions on $P_\Theta$ to Section~\ref{sec-fc-lower-stmt}.
We will denote by $f_{\expReward}$ the density of the element in $P_{\ExpRewards}$
with mean $\expReward$.

An \emph{infinite bandit model} is characterized by a probability measure
$\ArmMeasure$ over $(\Arms, \ArmEvents)$ together with a
measurable mapping $\ArmMean : \Arms \rightarrow \ExpRewards$
assigning a mean $\expReward$
(and therefore a reward distribution $p_\expReward$) to each arm.
The role of the measure $\ArmMeasure$ is to define the top-$\alpha$ fraction of arms, as we will show in Eq.~\ref{eq-good-arms};
it can be used by the algorithm to sample arms.
At each time step $t$, a user
%interacting with the bandit
selects an arm $\armRV_t \in \Arms$, based on past observation. He
can either query a new arm in $\Arms$
(which may be sampled $\armRV_t \sim \ArmMeasure$, or selected adaptively) or select an arm that
has been queried
in previous rounds. In any case, when arm $\armRV_t$ is drawn, an independent sample
$\rewardRV_t \sim p_{\ArmMean(\armRV_t)}$ is observed. 

For example, when boosting decision stumps
(binary classifiers which test a single feature against a threshold),
the set of arms $\Arms$ consists of all possible decision
stumps for the corpus, and
the expected reward for each arm is its expected accuracy over the sample space 
of all possible classification examples.
An algorithm may choose to draw the arms at random according to the
probability measure $\ArmMeasure$;
this is commonly done by, in effect, placing uniform probability mass over the
thresholds placed halfway between the distinct values seen in the training data
and placing zero mass over the remaining thresholds.
We are particularly interested in the case when the number of arms in the
support for $\ArmMeasure$ is so large as to be effectively infinite, at least with
respect to the available computational resources.

We denote by $\PrTrueModelNone$ and $\ETrueModelNone$ the probability and 
expectation under an infinite bandit model with arm probability measure
$\ArmMeasure$ and mean function $\ArmMean$. The
history of the bandit game up to time $t$ is
$\historyRV_t = ((\armRV_1,\rewardRV_1),\dots,(\armRV_t,\rewardRV_t)).$
By our assumption, the arm selected at round $t$ only depends on
$\historyRV_{t-1}$
and $U_t$, which is uniform on $[0,1]$ and independent of
$\historyRV_{t-1}$ (used to sample from $\ArmMeasure$ if needed).
In particular, the
conditional density of $\armRV_t$ given $\historyRV_{t-1}$,
denoted by  $\PrTrueModel{ \armRV_t | \historyRV_{t-1} }$,
is independent of the mean mapping $\ArmMean$. Note that this
property is
satisfied as well if, when querying a new arm, $\armRV_t$ can be chosen
arbitrarily 
in $\Arms$ (depending on $\historyRV_{t-1}$), and not necessarily at random from
$\ArmMeasure$. Under these
assumptions, one can compute the likelihood of $\historyRV_T$:
%
\vspace{-10pt}
%
\begin{align}
\ell\left(\historyRV_T ; \ArmMean,\ArmMeasure\right) = \prod_{t=1}^T f_{\ArmMean(\armRV_t)}(\rewardRV_t)
\PrTrueModel{ \armRV_t | \historyRV_{t-1} }.\label{Likelihood}
\end{align}
Note that the arms $\armRV_t$ are not latent objects: they are assumed to be
observed, but not their means $\ArmMean(\armRV_t)$.
For instance, in our text classification example we know the classifier we are
testing but not its true classification accuracy.
Treating arms as observed in this way simplifies the likelihood by making the
choice of new arms to query independent of their mean mappings.
This is key to our approach to dealing with reservoirs about which nothing
is known; we can avoid integrating over such reservoirs and so do not require
the reservoir to be smooth.

\subsection{Objective and Generic Algorithm}\label{generic}

\paragraph{Reservoir distribution.}
The probability space over arms $(\Arms, \ArmEvents, \ArmMeasure)$
and the mapping $\ArmMean$ is used to
form a pushforward measure over expected rewards
%\begin{align}
$
\ExpRewardMeasure(\cE) := (\ArmMean_*(\ArmMeasure))(\cE)
	= \ArmMeasure(\ArmMean^{-1}(\cE)), \text{ for } \cE \in \ExpRewardEvents,
$
%\end{align}
inducing the probability space
$(\ExpRewards, \ExpRewardEvents, \ExpRewardMeasure)$
over expected rewards.
We define our \emph{reservoir distribution} CDF
%\begin{align}
$
	\ExpRewardCDF(\tau) =
		\ExpRewardMeasure( \Set{\theta \le \tau} )
$
%\end{align}
whose density $\ExpRewardDensity$ is its Radon-Nikodym derivative
with respect to $\ArmMeasure$.
For convenience, we also define the ``inverse'' CDF
%\begin{align}
$
\ExpRewardInvCDF(p) := \inf \Set{ \expReward : G(\expReward) \ge p }.
$
%\end{align}
%
We assume that $G$ has bounded support and let
$\ArmMean^*$ be the largest possible mean under the reservoir distribution,
%\begin{align}
$
\ArmMean^* := \ExpRewardInvCDF(1)
	= \inf \Set{\expReward : G(\expReward) = 1 }.\label{eq-mustar}
$
%\end{align}

In the general setup introduced above, the reservoir may or may not be 
useful to query new arms, but it is needed to define the notion of top-$\alpha$
fraction.

\paragraph{Finding an arm in the top-$\alpha$ fraction.}
In our setting, for some fixed $\alpha \in ]0,1[$ and some $\epsilon \geq 0$, the goal is to identify an
arm that belongs to the set
\begin{align}\label{eq-good-arms}
\GTargetEps := \Set{
\arm \in \Arms :
\ArmMean(\arm) \ge \ExpRewardInvCDF(1 - \alpha) - \epsilon}
\end{align}
of arms whose expected mean rewards is high, in the sense that their mean is
within $\epsilon$ of
the quantile of order $1-\alpha$ of the reservoir distribution.
For notational convenience, when we set $\epsilon$ to zero we write 
$\GTargetNoEps := \GTargetZeroEps$.


% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-15pt}
% \begin{minipage}{0.4\textwidth}
% \begin{algorithm}[H]
% %
% \caption{Generic algorithm.}
% \label{algo:Generic}
% \begin{algorithmic}
% %
% \REQUIRE{Arm set $\Arms$, target $\alpha,\epsilon,\delta$}
% \ENSURE{Some arm $\hat{s}$}
% %
% \FOR{$t \gets 1,2,\dots$}
%  \STATE(choose one of:){
%  \begin{enumerate}
%  \item Pull arm: Choose $\armRV_t \sim \PrTrueModel{\armRV_t |
% H_{t-1}}$
%      and observe reward $\rewardRV_t \sim p_{\ArmMean(\armRV_t)}$
%  \item Stop: Choose $\hat{s} \gets \armRV_s$ for some $s < t$, \\
% 	{\textbf{return} $\hat{s}$} 
% \end{enumerate}
%  }
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \vspace{-15pt}
% \end{wrapfigure}

\paragraph{Generic algorithm}  An algorithm is made of a
\emph{sampling rule} $(\armRV_t)$, a \emph{stopping rule} $\tau$ (with
respect to the filtration generated by $\historyRV_t$) and a \emph{recommendation rule}
$\hat{s}_\tau$ that selects one of the queried arms as a candidate arm from
$\GTargetEps$. This is summarized in
Algorithm~\ref{algo:Generic}.


Fix $\delta \in ]0,1[$.
An algorithm that returns an arm from $\GTargetEps$
with probability at least $1-\delta$ is said to be
$(\alpha,\epsilon,\delta)$-correct.
Moreover, an $(\alpha,\epsilon,\delta)$-correct algorithm must perform
well on
all possible infinite bandit models:
%\begin{align*}
$
\forall (\ArmMeasure, \ArmMean), \ \
\PrTrueModel{ \hat{s}_\tau \in \GTargetEps }
	\geq 1 - \delta.
$
%\end{align*}
Our
goal is to build an $(\alpha,\epsilon,\delta)$-correct algorithm that uses as
few
samples as possible, i.e. for which $\ETrueModel{\tau}$ is small.
We similarly define the notion of $(\alpha,\delta)$-correctness
%in the case
when
$\epsilon=0$.


\paragraph{$(\alpha, \epsilon, \delta)$-correctness}
When little is known about the reservoir distribution
(e.g. it might not even be smooth), an $\epsilon$-relaxed algorithm is 
appropriate.
%It may be possible to estimate $\epsilon$ for arbitrary reservoirs, but we do
%not address this in the present work.
The choice of $\epsilon$ represents a tradeoff between simple regret
(defined shortly)
and the maximum budget used to differentiate between arms.
We provide our lower bound in both $\epsilon$-relaxed and unrelaxed forms.
Our algorithm requires an $\epsilon$ parameter, but we show how this parameter
can be chosen under regularity assumptions on the tail of the reservoir to
provide an $(\alpha,\delta)$-correct algorithm.


\paragraph{Simple regret guarantees.} In the infinite bandit literature,
performance is typically measured in
terms of
% the distance from the selected arm to the best mean of an arm under the
%reservoir,  called 
\emph{simple regret}: $r_\tau = \ArmMean^* - \ArmMean(\hat{s}_\tau)$.
%We argue here that
If the tail of the reservoir distribution is bounded, one
can obtain simple regret upper bounds for an
algorithm in our framework.

A classic assumption (see, e.g. \cite{DBLP:journals/corr/CarpentierV15}) is
that there
exists $\beta >0$ and two constants $E,E'$ such that
%
\vspace{-10pt}
%
\begin{align}
%$
\forall \rho >0,
	E\rho^\beta \leq \ExpRewardMeasure(\Set{\expReward
\geq \ArmMean^* - \rho})
	\leq E'\rho^\beta.\label{ass:smoothness}
%$
\end{align}
With $C = E^{-1/\beta}$ and $C'=(E')^{-1/\beta}$, this translates into 
%\begin{align*}
$
\forall \alpha >0, C\alpha^{1/\beta}
	\leq \ArmMean^* - \ExpRewardInvCDF(1-\alpha)
	\leq C' \alpha^{1/\beta},
$
%\end{align*}
and a $(\alpha,\delta)$-correct algorithm has its simple regret upper bounded as
%
\vspace{-10pt}
%
\begin{align}
\Pr{ r_\tau \leq C'\alpha^{1/\beta} } \geq 1-\delta.
\end{align}
Similarly, a $(\alpha,\epsilon,\delta)$-correct algorithm has its simple regret bounded
as
%
\vspace{-10pt}
%
\begin{align}
\Pr{ r_\tau \leq C'\alpha^{1/\beta} + \epsilon }
	\geq 1-\delta.
\end{align}
If
%the smoothness parameter
$\beta$ is known, $\alpha$ and $\epsilon$
can be chosen to guarantee a simple regret below an arbitrary bound.

==> preamble.tex <==
%\theoremstyle{plain}
%\newtheorem{claim}{\protect\claimname}
%\theoremstyle{plain}
%\newtheorem{prop}{\protect\propositionname}
%\theoremstyle{plain}
%\newtheorem{lem}{\protect\lemmaname}
%\theoremstyle{plain}
%\newtheorem{thm}{\protect\theoremname}
%\theoremstyle{plain}
%\newtheorem{cor}{\protect\corollaryname}  
%\theoremstyle{definition}
%\newtheorem{defn}{\protect\definitionname}
%\theoremstyle{definition}
%\newtheorem{assump}{\protect\assumptionname}
%\theoremstyle{definition}
%\newtheorem{rem}{\protect\remarkname}

\makeatother
  
\usepackage{babel} 

\providecommand{\claimname}{Claim}
\providecommand{\lemmaname}{Lemma}
\providecommand{\propositionname}{Proposition}
\providecommand{\theoremname}{Theorem}
\providecommand{\corollaryname}{Corollary} 
\providecommand{\definitionname}{Definition}
\providecommand{\assumptionname}{Assumption}
\providecommand{\remarkname}{Remark}

\newcommand{\overbar}[1]{\mkern 1.25mu\overline{\mkern-1.25mu#1\mkern-0.25mu}\mkern 0.25mu}
\newcommand{\overbarr}[1]{\mkern 3.5mu\overline{\mkern-3.5mu#1\mkern-0.75mu}\mkern 0.75mu}
\newcommand{\mytilde}[1]{\mkern 0.5mu\widetilde{\mkern-0.5mu#1\mkern-0mu}\mkern 0mu}
\newcommand{\mytildee}[1]{\mkern 1.5mu\widetilde{\mkern-1.5mu#1\mkern-0mu}\mkern 0mu}
  
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\minimize}{minimize} 
\newcommand{\openone}{\mathds{1}}

% \newcommand{\todo}[1]{{\bf \color{red} [TODO] #1 }}

% Robust GP
\newcommand{\Dbar}{\overbar{D}}
\newcommand{\Rbar}{\overbar{R}}
\newcommand{\Runder}{\underline{R}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\kSE}{k_{\text{SE}}}
\newcommand{\kMat}{k_{\text{Mat\'ern}}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ecbar}{\overbar{\mathcal{E}}}

% Other
\newcommand{\GP}{{\rm GP}}
\newcommand{\gv}{\mathbf{g}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\wv}{\mathbf{w}}
\newcommand{\zvbar}{\overbar{\mathbf{z}}}

% Ranking and bandits
\newcommand{\thetamin}{\theta_{\mathrm{min}}}
\newcommand{\thetamax}{\theta_{\mathrm{max}}}
\newcommand{\Xhat}{\widehat{X}}
\newcommand{\Ghat}{\widehat{G}}
\newcommand{\jworst}{j_{\mathrm{worst}}}
\newcommand{\Actil}{\widetilde{\mathcal{A}}}
% \newcommand{\Stil}{\widetilde{S}}
\newcommand{\mab}{\texttt{mab}}
\newcommand{\cmp}{\texttt{btl}}
\newcommand{\pemab}{P_{\mathrm{e},\texttt{mab}}}
\newcommand{\pecmp}{P_{\mathrm{e},\texttt{btl}}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\Alg}{\mathrm{ALG}}
\newcommand{\Geometric}{\mathrm{Geometric}}
\newcommand{\Ttotal}{T_{\mathrm{total}}}
\newcommand{\jsec}{j_{\mathrm{sec}}}

% NoisyDD
\newcommand{\NDhat}{\widehat{\mathrm{ND}}}
\newcommand{\PDhat}{\widehat{\mathrm{PD}}}
% \newcommand{\Dhat}{\widehat{\mathrm{D}}}
\newcommand{\Shat}{\widehat{S}}
\newcommand{\Ehat}{\widehat{E}}
\newcommand{\peid}{P_{\mathrm{e},1}^{(\mathrm{D})}}
\newcommand{\peind}{P_{\mathrm{e},1}^{(\mathrm{ND})}}
\newcommand{\peiid}{P_{\mathrm{e},2}^{(\mathrm{D})}}
\newcommand{\peiind}{P_{\mathrm{e},2}^{(\mathrm{ND})}}
\newcommand{\epsid}{\epsilon_{1}^{(\mathrm{D})}}
\newcommand{\epsind}{\epsilon_{1}^{(\mathrm{ND})}}
\newcommand{\epsiid}{\epsilon_{2}^{(\mathrm{D})}}
\newcommand{\epsiind}{\epsilon_{2}^{(\mathrm{ND})}}
\newcommand{\nid}{n_1^{(\mathrm{D})}}
\newcommand{\nind}{n_1^{(\mathrm{ND})}}
\newcommand{\niid}{n_2^{(\mathrm{D})}}
\newcommand{\niind}{n_2^{(\mathrm{ND})}}
\newcommand{\Npd}{N_{\mathrm{pos}}^{(\mathrm{D})}}
\newcommand{\Npnd}{N_{\mathrm{pos}}^{(\mathrm{ND})}}
\newcommand{\npd}{n_{\mathrm{pos}}^{(\mathrm{D})}}
\newcommand{\npnd}{n_{\mathrm{pos}}^{(\mathrm{ND})}}
\newcommand{\npos}{n_{\mathrm{pos}}}
\newcommand{\nneg}{n_{\mathrm{neg}}}
\newcommand{\Ntilpos}{\widetilde{N}_{\mathrm{pos}}}
% \newcommand{\Npos}{N_{\mathrm{pos}}}
% \newcommand{\Nneg}{N_{\mathrm{neg}}}
\newcommand{\Aid}{\mathcal{A}_{1,i}^{(\mathrm{D})}}
\newcommand{\Aind}{\mathcal{A}_{1,i}^{(\mathrm{ND})}}
\newcommand{\mutild}{\tilde{\mu}^{(\mathrm{D})}}
\newcommand{\mutilnd}{\tilde{\mu}^{(\mathrm{ND})}}

% OneDimBO

\newcommand{\diag}{\mathrm{diag}}
\newcommand{\cunder}{\underline{c}}
\newcommand{\cbar}{\overline{c}}
\newcommand{\mutil}{\widetilde{\mu}}
\newcommand{\sigmatil}{\widetilde{\sigma}}
\newcommand{\Tearly}{T_{\mathrm{early}}}
\newcommand{\Tlate}{T_{\mathrm{late}}}
\newcommand{\Rearly}{R_{\mathrm{early}}}
\newcommand{\Rlate}{R_{\mathrm{late}}}
\newcommand{\Ctil}{\widetilde{C}}
\newcommand{\ctil}{\widetilde{c}}
\newcommand{\ftil}{\widetilde{f}}
\newcommand{\UCB}{\mathrm{UCB}}
\newcommand{\LCB}{\mathrm{LCB}}
\newcommand{\UCBtil}{\widetilde{\mathrm{UCB}}}
\newcommand{\LCBtil}{\widetilde{\mathrm{LCB}}}
\newcommand{\Lctil}{\widetilde{\mathcal{L}}}

% NoisyAdaptiveGT

\newcommand{\nMIi}{n_{\mathrm{MI,1}}}
\newcommand{\nMIii}{n_{\mathrm{MI,2}}}
\newcommand{\nConc}{n_{\mathrm{Conc}}}
\newcommand{\nIndiv}{n_{\mathrm{Indiv}}}
\newcommand{\nHalving}{n_{\mathrm{Halving}}}
\newcommand{\kmax}{k_{\mathrm{max}}}
\newcommand{\ptil}{\widetilde{p}}
\newcommand{\elltil}{\widetilde{\ell}}
\newcommand{\Stil}{\widetilde{S}}
\newcommand{\ncheck}{\check{n}}

% SeparateGT

\newcommand{\cmean}{c_{\mathrm{mean}}}
\newcommand{\cvar}{c_{\mathrm{var}}}
\newcommand{\ccov}{c_{\mathrm{cov}}}
\newcommand{\cmax}{c_{\mathrm{max}}}

\newcommand{\dneg}{d_{\mathrm{neg}}}
\newcommand{\dpos}{d_{\mathrm{pos}}}
\newcommand{\Nneg}{N_{\mathrm{neg}}}
\newcommand{\Npos}{N_{\mathrm{pos}}}
\newcommand{\Nerr}{N_{\mathrm{err}}}
\newcommand{\alphaneg}{\alpha_{\mathrm{neg}}}
\newcommand{\alphapos}{\alpha_{\mathrm{pos}}}

\newcommand{\pej}{P_{\mathrm{e},j}}
\newcommand{\nusymm}{\nu_{\mathrm{symm}}}

% PooledData
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\Nrm}{\mathrm{N}}
\newcommand{\CNrm}{\mathrm{CN}}

% ConverseGP
\newcommand{\vbar}{\overline{v}}

% GT_ICASSP

\newcommand{\pc}{P_{\mathrm{c}}}

% ActiveMRF

\newcommand{\lammin}{\lambda_{\mathrm{min}}}
\newcommand{\lammax}{\lambda_{\mathrm{max}}}
\newcommand{\missing}{\ast}
\newcommand{\pFAi}{p_{\mathrm{FA},i}}
\newcommand{\pMDi}{p_{\mathrm{MD},i}}
\newcommand{\bSigmatil}{\widetilde{\mathbf{\Sigma}}}
\newcommand{\mtil}{\widetilde{m}}
\newcommand{\Ptil}{\widetilde{P}}
\newcommand{\dmin}{d_{\mathrm{min}}}
\newcommand{\davg}{d_{\mathrm{avg}}}
\newcommand{\dmaxbar}{\overline{d}_{\mathrm{max}}}
\newcommand{\taumin}{\tau_{\mathrm{min}}}
\newcommand{\taumax}{\tau_{\mathrm{max}}}
\newcommand{\ntil}{\widetilde{n}}
\newcommand{\Ntil}{\widetilde{N}}
\newcommand{\Ncheck}{\check{N}}
\newcommand{\kbar}{\overbar{k}}

\newcommand{\mmin}{m_{\mathrm{min}}}
\newcommand{\mmax}{m_{\mathrm{max}}}

% PartialSBM
\newcommand{\ellv}{\boldsymbol{\ell}}
\newcommand{\Cieq}{C_{1,\mathrm{eq}}}
\newcommand{\Cidif}{C_{1,\mathrm{dif}}}
\newcommand{\Ctilde}{\tilde{C}}
\newcommand{\dbar}{\overline{d}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\Poisson}{\mathrm{Poisson}}
\newcommand{\ktilde}{\tilde{k}}
 
% GT_ISIT
\newcommand{\Veq}{V_{\mathrm{eq}}}
\newcommand{\Vdif}{V_{\mathrm{dif}}}
\newcommand{\Vveq}{\mathbf{V}_{\mathrm{eq}}}
\newcommand{\Vvdif}{\mathbf{V}_{\mathrm{dif}}}
\newcommand{\veq}{v_{\mathrm{eq}}}
\newcommand{\vdif}{v_{\mathrm{dif}}}



%
% MultiMRI
%
\newcommand{\bpsi}{\boldsymbol{\psi}}


%
% Group testing 
%
\newcommand{\Hg}{\mathrm{Hypergeometric}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\dTV}{d_{\mathrm{TV}}}

%
% Graphical model selection
%
\newcommand{\Gbar}{\overbar{G}}
\newcommand{\Mbar}{\overbar{M}}
\newcommand{\qmax}{q_{\mathrm{max}}}

%
% Community detection
%
\newcommand{\Bi}{\mathrm{Binomial}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ev}{\mathbf{E}}

%
% Support recovery
%
\newcommand{\Sbar}{\overbar{S}}
\newcommand{\sbar}{\overbar{s}}

%\newcommand{\Wdif}{W_{\mathrm{dif}}}
%\newcommand{\Weq}{W_{\mathrm{eq}}}
%\newcommand{\wdif}{w_{\mathrm{dif}}}
%\newcommand{\weq}{w_{\mathrm{eq}}}

\newcommand{\Sdif}{S_{\mathrm{dif}}}
\newcommand{\Seq}{S_{\mathrm{eq}}}
\newcommand{\sdif}{s_{\mathrm{dif}}}
\newcommand{\sdifbar}{\overbar{s}_{\mathrm{dif}}}
\newcommand{\seqbar}{\overbar{s}_{\mathrm{eq}}}
\newcommand{\seq}{s_{\mathrm{eq}}}
\newcommand{\sdifhat}{\hat{s}_{\mathrm{dif}}}
\newcommand{\sdifx}{\overbar{s} \backslash s}
\newcommand{\seqx}{\overbar{s} \cap s}

\newcommand{\Xvdif}{\mathbf{X}_{\overbar{s} \backslash s}}
\newcommand{\Xveq}{\mathbf{X}_{\overbar{s} \cap s}}
\newcommand{\Xvdifo}{\mathbf{X}_{s \backslash \overbar{s}}}
\newcommand{\xvdif}{\mathbf{x}_{\overbar{s} \backslash s}}
\newcommand{\xveq}{\mathbf{x}_{\overbar{s} \cap s}}
\newcommand{\xveqo}{\mathbf{x}_{s \backslash \overbar{s}}}

\newcommand{\Ord}{\mathcal{O}}
\newcommand{\Yctil}{\widetilde{\mathcal{Y}}}

\newcommand{\dmax}{d_{\mathrm{max}}}
\newcommand{\dH}{d_{\mathrm{H}}}

\newcommand{\jeq}{j_{\mathrm{eq}}}
\newcommand{\jdiff}{j_{\mathrm{dif}}}

\newcommand{\Zhat}{\hat{Z}}
\newcommand{\Zhatmax}{\hat{Z}_{\mathrm{max}}}
\newcommand{\zdiff}{z_{\mathrm{dif}}}
\newcommand{\zcomm}{z_{\mathrm{eq}}}

\newcommand{\bmin}{b_{\mathrm{min}}}
\newcommand{\Bmin}{\beta_{\mathrm{min}}}
\newcommand{\bmax}{b_{\mathrm{max}}}
\newcommand{\sigbeta}{\sigma_{\beta}}
\newcommand{\siglv}{\sigma_{\sdif}}
%\newcommand{\Tr}{\mathrm{Tr}}

%\newcommand{\sign}{\mathrm{sign}}
\newcommand{\SNRdB}{\mathrm{SNR}_{\mathrm{dB}}}

\newcommand{\Weq}{W_{\mathrm{eq}}}
\newcommand{\Wdif}{W_{\mathrm{dif}}}
\newcommand{\weq}{w_{\mathrm{eq}}}
\newcommand{\wdif}{w_{\mathrm{dif}}}
\newcommand{\feq}{f_{\mathrm{eq}}}
\newcommand{\fdif}{f_{\mathrm{dif}}}

\newcommand{\bgood}{b_{\mathrm{good}}}
\newcommand{\bbad}{b_{\mathrm{bad}}}

\newcommand{\btil}{\widetilde{b}}
\newcommand{\betatil}{\widetilde{\beta}}
\newcommand{\betatileq}{\widetilde{\beta}_{\mathrm{eq}}}
\newcommand{\betatildif}{\widetilde{\beta}_{\mathrm{dif}}}
\newcommand{\btileq}{\widetilde{b}_{\mathrm{eq}}}
\newcommand{\btildif}{\widetilde{b}_{\mathrm{dif}}}
\newcommand{\stileq}{\widetilde{s}_{\mathrm{eq}}}
\newcommand{\stildif}{\widetilde{s}_{\mathrm{dif}}}
\newcommand{\pieq}{\pi_{\mathrm{eq}}}
\newcommand{\pidif}{\pi_{\mathrm{dif}}}
\newcommand{\Sdifhat}{\hat{S}_{\mathrm{dif}}}

\newcommand{\Bcfano}{\mathcal{B}'_{\mathrm{Fano}}}

\newcommand{\Sceq}{\mathcal{S}_{\mathrm{eq}}}
\newcommand{\Scdif}{\mathcal{S}_{\mathrm{dif}}}
\newcommand{\Nc}{\mathcal{N}}

%
% From MultiMRI
%
\newcommand{\Pv}{\mathbf{P}}
\newcommand{\Wvtil}{\widetilde{\mathbf{W}}}
\newcommand{\wtil}{\widetilde{w}}
\newcommand{\xvhat}{\hat{\mathbf{x}}}

%
% From Expanders_FOCS
%
\newcommand{\Bernoulli}{\mathrm{Bernoulli}}
\newcommand{\Binomial}{\mathrm{Binomial}}
\newcommand{\imtil}{\tilde{\imath}}
\newcommand{\SNR}{\mathrm{SNR}}

%
% From PaperBI
%
\newcommand{\CLM}{C_{\mathrm{LM}}}
\newcommand{\CSC}{C_{\mathrm{SC}}}
\newcommand{\ISC}{I_{\mathrm{SC}}}
\newcommand{\CM}{C_{\mathrm{M}}}
\newcommand{\Qmin}{Q_{\mathrm{min}}}
\newcommand{\Phat}{\widehat{P}}

%
% From JournalSU
%
\newcommand{\pebar}{\overbar{P}_{\mathrm{e}}}
\newcommand{\petilde}{\tilde{p}_{\mathrm{e}}}
\newcommand{\pe}{P_{\mathrm{e}}}
\newcommand{\pen}{P_{\mathrm{e},n}}
\newcommand{\peQ}{P_{\mathrm{e},Q}} 
\newcommand{\pemax}{P_{\mathrm{e},\mathrm{max}}} 
\newcommand{\msg}{\mathsf{m}}

\newcommand{\Ez}{E_{0}}
\newcommand{\Er}{E_{\mathrm{r}}}
\newcommand{\Esp}{E_{\mathrm{sp}}}
\newcommand{\Eziid}{E_{0}^{\mathrm{iid}}}
\newcommand{\Ezcc}{E_{0}^{\mathrm{cc}}}
\newcommand{\Eohatcc}{\hat{E}_{0}^{\mathrm{cc}}}
\newcommand{\Eohatcost}{\hat{E}_{0}^{\mathrm{cost}}}
\newcommand{\Ezcost}{E_{0}^{\mathrm{cost}}}
\newcommand{\Ezcostprime}{E_{0}^{\mathrm{cost}^{\prime}}}
\newcommand{\Eriid}{E_{\mathrm{r}}^{\mathrm{iid}}}
\newcommand{\Ercc}{E_{\mathrm{r}}^{\mathrm{cc}}}
\newcommand{\Erccprime}{E_{\mathrm{r},12}^{\mathrm{cc}^{\prime}}}
\newcommand{\Ercost}{E_{\mathrm{r}}^{\mathrm{cost}}}
\newcommand{\Ercostprime}{E_{\mathrm{r}}^{\mathrm{cost}^{\prime}}}

\newcommand{\rcu}{\mathrm{rcu}}
\newcommand{\rcus}{\rcu_{s}}
\newcommand{\rcuss}{\rcu_{s}^{*}}
\newcommand{\rcusa}{\rcu_{s,a}^{*}}
\newcommand{\rcushat}{\widehat{\mathrm{rcu}}_{s}}
\newcommand{\rcusshat}{\widehat{\mathrm{rcu}}_{s}^{*}}
\newcommand{\alphasa}{\alpha^{\mathrm{iid}}}
\newcommand{\rcul}{\rcu_{\mathrm{L}}}
\newcommand{\rhohat}{\hat{\rho}}
\newcommand{\LM}{I_{\mathrm{LM}}}
\newcommand{\GMI}{I_{\mathrm{GMI}}}

\newcommand{\SetScc}{\mathcal{S}}
\newcommand{\SetSncc}{\mathcal{S}_{n}}
\newcommand{\SetSncost}{\mathcal{S}_{n}}
\newcommand{\SetSiid}{\mathcal{S}^{\mathrm{iid}}}
\newcommand{\SetScost}{\mathcal{S}}
\newcommand{\SetSniid}{\mathcal{S}_{n}^{\mathrm{iid}}}
\newcommand{\SetTcc}{\mathcal{T}}
\newcommand{\SetTiid}{\mathcal{T}^{\mathrm{iid}}}
\newcommand{\SetTcost}{\mathcal{T}}
\newcommand{\SetTncost}{\mathcal{T}_{n}}
\newcommand{\SetTncc}{\mathcal{T}_{n}}

\newcommand{\Miid}{M^{\mathrm{iid}}}
\newcommand{\Mcc}{M^{\mathrm{cc}}}
\newcommand{\Mcost}{M^{\mathrm{cost}}}
\newcommand{\Rcr}{R_{\mathrm{cr}}}
\newcommand{\Rcrs}{R_s^{\mathrm{cr}}}

\newcommand{\Fbar}{\overbar{F}}
\newcommand{\Funder}{\underline{F}}
\newcommand{\Gunder}{\underline{G}}
\newcommand{\PXv}{P_{\Xv}}
\newcommand{\qbar}{\overbar{q}}
\newcommand{\rbar}{\overbar{r}}
\newcommand{\rtilde}{\tilde{r}}
\newcommand{\atilde}{\tilde{a}}
\newcommand{\phitilde}{\tilde{\phi}}
\newcommand{\Mtilde}{\mytildee{M}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Rtilde}{\mytildee{R}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Wvtilde}{\widetilde{\mathbf{W}}}
\newcommand{\hover}{\overbar{h}}
\newcommand{\ubar}{\overbar{u}}
\newcommand{\Ubar}{\overbar{U}}
\newcommand{\xbarbar}{\overbar{\overbar{x}}}
\newcommand{\Xbarbar}{\overbar{\overbar{X}}}
\newcommand{\xbar}{\overbar{x}}
\newcommand{\Xbar}{\overbar{X}}
\newcommand{\xtilde}{\widetilde{x}}
\newcommand{\Xtilde}{\mytilde{X}}
\newcommand{\ybar}{\overbar{y}}
\newcommand{\zbar}{\overbar{z}}
\newcommand{\Zbar}{\overbar{Z}}
\newcommand{\thetabar}{\overbar{\theta}}

\newcommand{\av}{\mathbf{a}}
\newcommand{\Qv}{\mathbf{Q}}
\newcommand{\uvbar}{\overbar{\mathbf{u}}}
\newcommand{\uv}{\mathbf{u}}
\newcommand{\Uvbar}{\overbar{\mathbf{U}}}
\newcommand{\Uv}{\mathbf{U}}
%\newcommand{\vv}{\mathbf{v}}
\newcommand{\Vv}{\mathbf{V}}
\newcommand{\vvbar}{\overbar{\mathbf{v}}}
\newcommand{\xvbarbar}{\overbar{\overbar{\mathbf{x}}}}
\newcommand{\xvbar}{\overbar{\mathbf{x}}}
\newcommand{\xvtilde}{\widetilde{\mathbf{x}}}
\newcommand{\xv}{\mathbf{x}}
\newcommand{\Xvbarbar}{\overbar{\overbar{\mathbf{X}}}}
\newcommand{\Xvbar}{\overbar{\mathbf{X}}}
\newcommand{\Xvtilde}{\mytilde{\mathbf{X}}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Yvtilde}{\widetilde{\mathbf{Y}}}
\newcommand{\Xv}{\mathbf{X}}
\newcommand{\yv}{\mathbf{y}}
\newcommand{\Yv}{\mathbf{Y}}
\newcommand{\zv}{\mathbf{z}}
\newcommand{\Zv}{\mathbf{Z}}

\newcommand{\Yvs}{\mathbf{Y}_{\hspace*{-0.5ex}s}}
\newcommand{\Uvn}{\mathbf{U}_{\hspace*{-0.3ex}n}}
\newcommand{\Tvn}{\mathbf{T}_{\hspace*{-0.3ex}n}} 
\newcommand{\Vvi}{\mathbf{V}_{\hspace*{-0.3ex}1}} 
\newcommand{\Vvii}{\mathbf{V}_{\hspace*{-0.3ex}2}}
\newcommand{\Vvm}{\mathbf{V}_{\hspace*{-0.3ex}m}}
\newcommand{\Vvtilden}{\widetilde{\mathbf{V}}_{\hspace*{-0.3ex}n}}   
\newcommand{\QUn}{Q_{U\hspace*{-0.2ex},\hspace*{0.05ex}n}}
\newcommand{\QXgUn}{Q_{X|U\hspace*{-0.2ex},\hspace*{0.05ex}n}}
\newcommand{\QUXn}{Q_{UX\hspace*{-0.2ex},\hspace*{0.05ex}n}}
\newcommand{\Yvi}{\mathbf{Y}_{\hspace*{-0.5ex}1}}
\newcommand{\Yvii}{\mathbf{Y}_{\hspace*{-0.5ex}2}}
\newcommand{\Yvu}{\mathbf{Y}_{\hspace*{-0.5ex}u}}

\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\ic}{\mathcal{i}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}

\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\Qsf}{\mathsf{Q}}

%\newcommand{\al}{\{a_l\}}
%\newcommand{\rl}{\{r_l\}}
\newcommand{\rbarl}{\{\overbar{r}_l\}}
\newcommand{\defeq}{\triangleq}
\newcommand{\deq}{\stackrel{d}{=}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\erfcxi}{\mathrm{erfcx}_{1}}
\newcommand{\erfcx}{\mathrm{erfcx}}
\newcommand{\erfc}{\mathrm{erfc}}
\newcommand{\supp}{\mathrm{supp}}

\newcommand{\alphanl}{\alpha^{\mathrm{nl}}_n}
\newcommand{\alphal}{\alpha^{\mathrm{l}}_n}
\newcommand{\betanl}{\beta^{\mathrm{nl}}_n}
\newcommand{\betal}{\beta^{\mathrm{l}}_n}

\newcommand{\Es}{E_{\mathrm{s}}}
\newcommand{\EJ}{E_{\mathrm{J}}}
\newcommand{\EJi}{E_{\mathrm{J},1}}
\newcommand{\EJii}{E_{\mathrm{J},2}}

\newcommand{\Vmin}{V_{\mathrm{min}}}
\newcommand{\Vmax}{V_{\mathrm{max}}}

%
% From PaperExpurgated
%

\newcommand{\rcux}{\mathrm{rcux}}

\newcommand{\Eexiid}{E_{\mathrm{ex}}^{\mathrm{iid}}}
\newcommand{\Eexcc}{E_{\mathrm{ex}}^{\mathrm{cc}}}
\newcommand{\Eexhatcc}{\hat{E}_{\mathrm{ex}}^{\mathrm{cc}}}
\newcommand{\Eexcost}{E_{\mathrm{ex}}^{\mathrm{cost}}}
\newcommand{\Eexcostprime}{E_{\mathrm{ex}}^{\mathrm{cost}^{\prime}}}
\newcommand{\Exiid}{E_{\mathrm{x}}^{\mathrm{iid}}}
\newcommand{\Excc}{E_{\mathrm{x}}^{\mathrm{cc}}}
\newcommand{\Excost}{E_{\mathrm{x}}^{\mathrm{cost}}}
\newcommand{\Excoststar}{E_{\mathrm{x}}^{\mathrm{cost}^{*}}}
\newcommand{\Excostprime}{E_{\mathrm{x}}^{\mathrm{cost}^{\prime}}}
\newcommand{\Eex}{E_{\mathrm{ex}}}
\newcommand{\Ex}{E_{\mathrm{x}}}

\newcommand{\Pxbicm}{P_{X}^{\rm bicm}}

\newcommand{\Av}{\mathbf{A}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\mbar}{\overbar{m}}
\newcommand{\tv}{\mathbf{t}}

\newcommand{\Lsf}{\mathsf{L}}
\newcommand{\Csf}{\mathsf{C}}
\newcommand{\csf}{\mathsf{c}}
\newcommand{\Fsf}{\mathsf{F}}
\newcommand{\Tsf}{\mathsf{T}}

\newcommand{\brl}{\{\overbar{r}_l\}}

%
% From DocumentMU
%

\newcommand{\peobar}{\overbar{p}_{\mathrm{e},0}}
\newcommand{\peibar}{\overbar{p}_{\mathrm{e},1}}
\newcommand{\peiibar}{\overbar{p}_{\mathrm{e},2}}
\newcommand{\peiiibar}{\overbar{p}_{\mathrm{e},12}}
\newcommand{\peo}{P_{\mathrm{e},0}}
\newcommand{\pei}{P_{\mathrm{e},1}}
\newcommand{\peii}{P_{\mathrm{e},2}}
\newcommand{\peiii}{P_{\mathrm{e},12}}
\newcommand{\rcuo}{\mathrm{rcu}_{0}}
\newcommand{\rcui}{\mathrm{rcu}_{1}}
\newcommand{\rcuii}{\mathrm{rcu}_{2}}
\newcommand{\rcuiii}{\mathrm{rcu}_{12}}
\newcommand{\rcuiiiprime}{\mathrm{rcu}_{12}^{\prime}}
\newcommand{\rcuiiia}{\mathrm{rcu}_{12,1}}
\newcommand{\rcuiiib}{\mathrm{rcu}_{12,2}}

\newcommand{\Eiziid}{E_{0,1}^{\mathrm{iid}}}
\newcommand{\Eiiziid}{E_{0,2}^{\mathrm{iid}}}
\newcommand{\Eiiiziid}{E_{0,12}^{\mathrm{iid}}}
\newcommand{\Eiiiaziid}{E_{0,12,1}^{\mathrm{iid}}}
\newcommand{\Eiiibziid}{E_{0,12,2}^{\mathrm{iid}}}
\newcommand{\Eozcc}{E_{0,0}^{\mathrm{cc}}}
\newcommand{\Eizcc}{E_{0,1}^{\mathrm{cc}}}
\newcommand{\Eiizcc}{E_{0,2}^{\mathrm{cc}}}
\newcommand{\Eiiizcc}{E_{0,12}^{\mathrm{cc}}}
\newcommand{\Eiiizccprime}{E_{0,12}^{\mathrm{cc}^{\prime}}}
\newcommand{\Eiiizccpprime}{E_{0,12}^{\mathrm{cc}^{\prime\prime}}}
\newcommand{\Eiiiazcc}{E_{0,12,1}^{\mathrm{cc}}}
\newcommand{\Eiiibzcc}{E_{0,12,2}^{\mathrm{cc}}}
\newcommand{\Ehatiiiazcc}{\hat{E}_{0,12,1}^{\mathrm{cc}}}
\newcommand{\Eozcost}{E_{0,0}^{\mathrm{cost}}}
\newcommand{\Eizcost}{E_{0,1}^{\mathrm{cost}}}
\newcommand{\Eiizcost}{E_{0,2}^{\mathrm{cost}}}
\newcommand{\Eiiizcost}{E_{0,12}^{\mathrm{cost}}}
\newcommand{\Eiiiazcost}{E_{0,12,1}^{\mathrm{cost}}}
\newcommand{\Eiiibzcost}{E_{0,12,2}^{\mathrm{cost}}}
\newcommand{\Eiiizaccts}{E_{0,12,1}^{\text{cc-ts}}}

\newcommand{\Eiriid}{E_{\mathrm{r},1}^{\mathrm{iid}}}
\newcommand{\Eiiriid}{E_{\mathrm{r},2}^{\mathrm{iid}}}
\newcommand{\Eiiiriid}{E_{\mathrm{r},12}^{\mathrm{iid}}}
\newcommand{\Eiiiariid}{E_{\mathrm{r},12,1}^{\mathrm{iid}}}
\newcommand{\Eiiibriid}{E_{\mathrm{r},12,2}^{\mathrm{iid}}}
\newcommand{\Eorcc}{E_{\mathrm{r},0}^{\mathrm{cc}}}
\newcommand{\Eorccprime}{E_{\mathrm{r},0}^{\mathrm{cc}^{\prime}}}
\newcommand{\Eircc}{E_{\mathrm{r},1}^{\mathrm{cc}}}
\newcommand{\Eiircc}{E_{\mathrm{r},2}^{\mathrm{cc}}}
\newcommand{\Eiiircc}{E_{\mathrm{r},12}^{\mathrm{cc}}}
\newcommand{\Eiiiarcc}{E_{\mathrm{r},12,1}^{\mathrm{cc}}}
\newcommand{\Eiiibrcc}{E_{\mathrm{r},12,2}^{\mathrm{cc}}}
\newcommand{\Eorcost}{E_{\mathrm{r},0}^{\mathrm{cost}}}
\newcommand{\Eircost}{E_{\mathrm{r},1}^{\mathrm{cost}}}
\newcommand{\Eiircost}{E_{\mathrm{r},2}^{\mathrm{cost}}}
\newcommand{\Eiiircost}{E_{\mathrm{r},12}^{\mathrm{cost}}}
\newcommand{\Eiiiarcost}{E_{\mathrm{r},12,1}^{\mathrm{cost}}}
\newcommand{\Eiiibrcost}{E_{\mathrm{r},12,2}^{\mathrm{cost}}}
\newcommand{\Eiiirtilde}{\widetilde{E}_{\mathrm{r,12}}}
\newcommand{\Eiiirccts}{E_{\mathrm{r},12}^{\text{cc-ts}}}

\newcommand{\Wsu}{W^{\prime}}
\newcommand{\qsu}{q^{\prime}}
\newcommand{\RegLM}{\mathcal{R}_{\mathrm{LM}}}
\newcommand{\RegLMex}{\mathcal{R}_{\mathrm{ex}}}

\newcommand{\SetSccts}{\mathcal{S}^{\mathrm{ts}}}
\newcommand{\SetTocc}{\mathcal{T}_0}
\newcommand{\SetToncc}{\mathcal{T}_{0,n}}
\newcommand{\SetTicc}{\mathcal{T}_{1}}
\newcommand{\SetTiicc}{\mathcal{T}_{2}}
\newcommand{\SetTiiicc}{\mathcal{T}_{12}}
\newcommand{\SetTiiincc}{\mathcal{T}_{12,n}}
\newcommand{\SetTnucc}{\mathcal{T}_{\nu}}
\newcommand{\SetTnuccex}{\mathcal{T}_{\nu}^{\mathrm{ex}}}
\newcommand{\SetTiccex}{\mathcal{T}_{1}^{\mathrm{ex}}}
\newcommand{\SetTiiccex}{\mathcal{T}_{2}^{\mathrm{ex}}}
\newcommand{\SetTiiiccex}{\mathcal{T}_{12}^{\mathrm{ex}}}
\newcommand{\SetTiccts}{\mathcal{T}_{1}^{\mathrm{ts}}}
\newcommand{\SetTiiccts}{\mathcal{T}_{2}^{\mathrm{ts}}}
\newcommand{\SetTiiiccts}{\mathcal{T}_{12}^{\mathrm{ts}}}

\newcommand{\qv}{\mathbf{q}}
\newcommand{\Wv}{\mathbf{W}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Vc}{\mathcal{V}}

\newcommand{\Rsc}{R^{\mathrm{sc}}}
\newcommand{\Rmac}{R^{\mathrm{ex}}}
\newcommand{\Rosc}{R_{0}^{\mathrm{sc}}}
\newcommand{\Risc}{R_{1}^{\mathrm{sc}}}
\newcommand{\Rimac}{R_{1}^{\mathrm{ex}}}
\newcommand{\Riimac}{R_{2}^{\mathrm{ex}}}
\newcommand{\Usc}{U^{\mathrm{sc}}}
\newcommand{\Ucsc}{\mathcal{U}^{\mathrm{sc}}}
\newcommand{\Ximac}{X_{1}^{\mathrm{ex}}}
\newcommand{\Xcimac}{\mathcal{X}_{1}^{\mathrm{ex}}}
\newcommand{\Xiimac}{X_{2}^{\mathrm{ex}}}
\newcommand{\Xciimac}{\mathcal{X}_{2}^{\mathrm{ex}}}

\newcommand{\PrML}{\PP^{(\mathrm{ML})}}
\newcommand{\PrS}{\PP^{(\mathrm{S})}}
\newcommand{\PrGenie}{\PP^{(\mathrm{Genie})}}

%
% From MAC2OR
%
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\cv}{\mathbf{c}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Iv}{\mathbf{I}}
\newcommand{\iv}{\mathbf{i}}
\newcommand{\Fv}{\mathbf{F}}
\newcommand{\fv}{\mathbf{f}}
\newcommand{\Mv}{\mathbf{M}}
\newcommand{\Jv}{\mathbf{J}}
\newcommand{\Kv}{\mathbf{K}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\Lv}{\mathbf{L}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\sv}{\mathbf{s}}
\newcommand{\Sv}{\mathbf{S}}
\newcommand{\Tv}{\mathbf{T}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\bone}{\boldsymbol{1}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bell}{\boldsymbol{\ell}}
\newcommand{\Qinv}{\mathsf{Q}_{\mathrm{inv}}}

%
% From RefinementCC
%
\newcommand{\Wocc}{\mathcal{W}_{0}^{\mathrm{cc}}}
\newcommand{\Wosymm}{\mathcal{W}_{0}^{\mathrm{symm}}}
\newcommand{\Wsymm}{\mathcal{W}^{\mathrm{symm}}}
\newcommand{\Qocc}{\mathcal{Q}_{0}^{\mathrm{cc}}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\Ezxcc}{E_{0,x}^{\mathrm{cc}}}
\newcommand{\Ezxicc}{E_{0,x_{i}}^{\mathrm{cc}}}
\newcommand{\Rcrsa}{R_{s,a}^{\mathrm{cr}}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
